Graph Inverse Reinforcement Learning from Diverse Videos

Research on Inverse Reinforcement Learning (IRL) from third-person videos has shown encouraging results on removing the need for manual reward design for robotic tasks. However, most prior works are still limited by training from a relatively restricted domain of videos. In this paper, we argue that the true potential of third-person IRL lies in increasing the diversity of videos for better scaling. To learn a reward function from diverse videos, we propose to perform graph abstraction on the videos followed by temporal matching in the graph space to measure the task progress. Our insight is that a task can be described by entity interactions that form a graph, and this graph abstraction can help remove irrelevant information such as textures, resulting in more robust reward functions. We evaluate our approach, GraphIRL, on cross-embodiment learning in X-MAGICAL and learning from human demonstrations for real-robot manipulation. We show significant improvements in robustness to diverse video demonstrations over previous approaches, and even achieve better results than manual reward design on a real robot pushing task. Videos are available at https://sateeshkumar21.github.io/GraphIRL .

==> tables/robot-simulation-final-distance.tex <==
\begin{table*}[ht!]
\begin{minipage}[c]{1.0 \textwidth}
\centering

\begin{tabular}{lccccccc}

\specialrule{1pt}{1pt}{1pt}

\textit{Simulation}  &  {XIRL} & {TCN} & {LIFS} & {Env. Reward} & {GIL (Ours)}\\
% 
\midrule
%Push (Mujoco)	& - & - &	- & - & - \\
Push & $0.224 \scriptstyle{\pm 0.051}$ & - & - & $0.138 \scriptstyle{\pm 0.041}$ & $\mathbf{0.083 \scriptstyle{\pm 0.009}}$ \\
Reach & $0.0515  \scriptstyle{\pm 0.005}$& $0.164  \scriptstyle{\pm 0.058}$ & $0.1415  \scriptstyle{\pm 0.014}$ & $0.007  \scriptstyle{\pm 0.002} $ & $\mathbf{0.006  \scriptstyle{\pm 0.002}}$ \\
Peg-in-box & - & - & - & - & -\\

%OT+CTE & 34.3 &	40.4 \\


\specialrule{1pt}{1pt}{1pt}
\end{tabular}

\caption{Final distance between goal and object on robot manipulation tasks in simulation. Average and standard error over 5 seeds. Lower is better.}
\label{tab:robot_sim_distance}
\end{minipage}\hfill
\end{table*}

==> tables/robot-simulation.tex <==
\begin{table*}[t]
\begin{minipage}[c]{1.0 \textwidth}
\centering
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{lccccccc}

\specialrule{1pt}{1pt}{1pt}

\textit{Simulation}  &  {XIRL} & {TCN} & {LIFS} & {Env. Reward} & {GraphIRL (Ours)}\\
% 
\midrule
%Push (Mujoco)	& - & - &	- & - & - \\
Push & $0.187 \scriptstyle{\pm 0.066}$ & $0.155 \scriptstyle{\pm 0.071}$ & $0.075 \scriptstyle{\pm 0.019}$ & $0.512 \scriptstyle{\pm 0.228}$ & $0.832 \scriptstyle{\pm 0.039}$ \\
Reach & $0.477  \scriptstyle{\pm 0.056}$& $0.14 \scriptstyle{\pm 0.1}$ & $0.0933 \scriptstyle{\pm 0.04}$& $1.0$ & $1.0$ \\
Peg in Box &  $0.000 \scriptstyle{\pm 0.000}$ &  $0.000 \scriptstyle{\pm 0.000}$ & $0.000 \scriptstyle{\pm 0.000}$  & $0.38 \scriptstyle{\pm 0.358} $ & $0.42  \scriptstyle{\pm 0.263}$ \\
\specialrule{1pt}{1pt}{1pt}
\end{tabular}
}
\caption{\textbf{Robotic Manipulation.} Success rates of our method \emph{GraphIRL} and baselines on the tasks of \emph{Reach}, \emph{Push} and \emph{Peg-in-box}. All results are averaged over 5 seeds. We observe significant gains in performance specially over vision-based baselines due to large \emph{domain-gap}.}
\vspace{-0.1in}
\label{tab:robot_sim_goal}
\end{minipage}\hfill
\end{table*}

==> tables/xmagical-old/xmagical-cross-env-cross-emb.tex <==
\begin{table}[!ht]
\begin{minipage}[c]{0.48\linewidth}
% =\centering
\begin{tabular}{l|ccc|c}
\specialrule{1pt}{1pt}{1pt}

Embodiment  &  {XIRL} & {TCN} & {LIFS} & {GIL} \\
% 
\midrule
Gripper	&  $0.373 \scriptstyle{\pm 0.021}$ & - & - & 0.729 \\
Short-stick &  $0.447 \scriptstyle{\pm 0.042}$ & - & - & 0.540 \\
Medium-stick & - & - & - & 0.912 \\
Long-stick & $0.532 \scriptstyle{\pm 0.470}$ & - & - & 0.919 \\


\specialrule{1pt}{1pt}{1pt}
\end{tabular}

\caption{Success rate on X-MAGICAL under Cross-Environment Cross-Embodiment Setting. Pretraining on \underline{Standard} and RL on \underline{Diverse}}
\label{tab:xmag_rand_std_rl_rand}
\vspace{-0.6cm}
\end{minipage}\hfill

\begin{minipage}[c]{0.48\linewidth}
\centering
\begin{tabular}{l|ccc|c}

\specialrule{1pt}{1pt}{1pt}

Embodiment  &  {XIRL} & {TCN} & {LIFS} & {GIL}\\
% 
\midrule
Gripper	& $0.439 \scriptstyle{\pm 0.335}$ & - & - & 0.571 \\
Short-stick &  $0.512 \scriptstyle{\pm 0.055}$ & - & - & 0.541 \\
Medium-stick &  $0.888 \scriptstyle{\pm 0.057}$ & - & - & 0.871 \\
Long-stick &  $0.993 \scriptstyle{\pm 0.009}$ & - & - & 0.981 \\


\specialrule{1pt}{1pt}{1pt}
\end{tabular}
\caption{Success rate on X-MAGICAL under Cross-Environment Cross-Embodiment Setting. Pretraining on \underline{Diverse} and RL on \underline{Standard}}
\label{tab:ablation_yti}
\vspace{-0.6cm}
\end{minipage}
\end{table}

==> tables/xmagical-old/xmagical-cross-env-same-emb.tex <==
\begin{table}[!ht]
\begin{minipage}[c]{0.48\linewidth}
% \centering
\begin{tabular}{l|ccc|c}

\specialrule{1pt}{1pt}{1pt}

Embodiment  &  {XIRL} & {TCN} & {LIFS} & {GIL} \\
% 
\midrule
Gripper	&  $0.627 \scriptstyle{\pm 0.033}$ & - & - & - \\
Short-stick &  $0.275 \scriptstyle{\pm 0.206}$ & - & - & - \\
Medium-stick & - & - & - & - \\
Long-stick & $0.779 \scriptstyle{\pm 0.406}$ & - & - & - \\


\specialrule{1pt}{1pt}{1pt}
\end{tabular}

\caption{Success rate on X-MAGICAL under Cross-Environment Setting. Pretraining on \underline{Standard} and RL on \underline{Diverse}}
\label{tab:xmag_rand_std_rl_rand}
\vspace{-0.6cm}
\end{minipage}\hfill

\begin{minipage}[c]{0.48\linewidth}
\centering
\begin{tabular}{l|ccc|c}

\specialrule{1pt}{1pt}{1pt}

Embodiment  &  {XIRL} & {TCN} & {LIFS} & {GIL}\\
% 
\midrule
Gripper	& $0.499 \scriptstyle{\pm 0.416}$ & - & - & - \\
Short-stick &  $0.496 \scriptstyle{\pm 0.054}$ & - & - & - \\
Medium-stick &  $0.944 \scriptstyle{\pm 0.027}$ & - & - & - \\
Long-stick &  $0.583 \scriptstyle{\pm 0.464}$ & - & - & - \\


\specialrule{1pt}{1pt}{1pt}
\end{tabular}
\caption{Success rate on X-MAGICAL under Cross-Environment Same-Embodiment Setting. Pretraining on \underline{Diverse} and RL on \underline{Standard}}
\label{tab:ablation_yti}
\vspace{-0.6cm}
\end{minipage}
\end{table}

==> tables/xmagical-old/xmagical-same-env-cross-emb.tex <==
\begin{table}[!ht]
\begin{minipage}[c]{0.48\linewidth}
% \centering
\begin{tabular}{l|ccc|c}

\specialrule{1pt}{1pt}{1pt}

Embodiment  &  {XIRL} & {TCN} & {LIFS} & {GIL}\\
% 
\midrule
Gripper	& $0.404 \scriptstyle{\pm 0.042}$ &	- & - & 0.741  \\
Short-stick & $0.619 \scriptstyle{\pm 0.030}$ & - & - & 0.677 \\
Medium-stick & $0.789 \scriptstyle{\pm 0.032}$ & - & - &  0.895 \\
Long-stick & $0.960 \scriptstyle{\pm 0.062}$  & - & - &  0.996 \\


\specialrule{1pt}{1pt}{1pt}
\end{tabular}

\caption{Success rate on X-MAGICAL under Same-Environment Cross-Embodiment Setting. Pretraining on \underline{Standard} and RL on \underline{Standard}}
\label{tab:xmag_pre_std_rl_std}

\end{minipage}\hfill
\begin{minipage}[c]{0.48\linewidth}
\centering
\begin{tabular}{l|ccc|c}

\specialrule{1pt}{1pt}{1pt}

Embodiment  &  {XIRL} & {TCN} & {LIFS} & {GIL}\\
% 
\midrule
Gripper & $0.703 \scriptstyle{\pm 0.056}$ & 	- & - & 0.614 \\
Short-stick &  $0.533 \scriptstyle{\pm 0.051}$ & - & - & 0.451 \\
Medium-stick &  $0.904 \scriptstyle{\pm 0.011}$ & - & - & 0.844 \\
Long-stick &  $0.713 \scriptstyle{\pm 0.444}$ & - & - & 0.868 \\


\specialrule{1pt}{1pt}{1pt}
\end{tabular}
\caption{Success rate on X-MAGICAL under Same-Environment Cross-Embodiment Setting. Pretraining on \underline{Diverse} and RL on \underline{Diverse}}
\label{tab:xmag_pre_rand_rl_rand}

\end{minipage}
\end{table}

==> tables/xmagical/cross-emb-cross-env.tex <==
\begin{table*}[ht!]
\label{tab:cross-emb-cross-env}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccc|c}
\multicolumn{1}{c}{} & \multicolumn{3}{c}{} & \multicolumn{1}{c}{} \\
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Standard Env. Pretraining $\rightarrow$ Diverse Env. RL} & \multicolumn{1}{c}{} \\
\toprule
Emb & XIRL & TCN & LIFS & \textbf{GIL} (Ours) \\\midrule
Gripper	&  $0.34 \scriptstyle{\pm 0.04}$ & - & - & $\mathbf{0.729}$ \\
S-stick &  $0.40 \scriptstyle{\pm 0.03}$ & $0.33 \scriptstyle{\pm 0.07}$ & $0.33 \scriptstyle{\pm 0.07}$ & $\mathbf{0.540}$ \\
M-stick & $0.64 \scriptstyle{\pm 0.14}$ & - & - & $\mathbf{0.912}$ \\
L-stick & $0.54 \scriptstyle{\pm 0.47}$ & $0.31 \scriptstyle{\pm 0.06}$ & $0.31 \scriptstyle{\pm 0.06}$ & $\mathbf{0.919}$ \\
\bottomrule
\end{tabular}
\hspace{1em}
\begin{tabular}{l|ccc|c}
\multicolumn{1}{c}{} & \multicolumn{3}{c}{} & \multicolumn{1}{c}{} \\
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Diverse Env. Pretraining $\rightarrow$ Standard Env. RL} & \multicolumn{1}{c}{} \\
\toprule
Emb. & XIRL & TCN & LIFS & \textbf{GIL} (Ours) \\\midrule
Gripper	& $\mathbf{0.70 \scriptstyle{\pm 0.06}}$ & $0.00 \scriptstyle{\pm 0.00}$ & $0.00 \scriptstyle{\pm 0.00}$ & $0.571$ \\
S-stick &  $0.51 \scriptstyle{\pm 0.23}$ & $0.00 \scriptstyle{\pm 0.00}$ & $0.00 \scriptstyle{\pm 0.00}$ & $\mathbf{0.541}$ \\
M-stick &  $0.71 \scriptstyle{\pm 0.39}$ & $0.00 \scriptstyle{\pm 0.00}$ & $0.00 \scriptstyle{\pm 0.00}$ & $\mathbf{0.871}$ \\
L-stick &  $\mathbf{0.99 \scriptstyle{\pm 0.01}}$ & $0.01 \scriptstyle{\pm 0.01}$ & $0.01 \scriptstyle{\pm 0.01}$ & $0.981$ \\
\bottomrule
\end{tabular}
}
\caption{\textit{\textbf{Cross-Embodiment Cross-Environment:}} We benchmark the cross-environment cross-embodiment performance of XIRL, TCN, and LIFS alongside GIL for the X-MAGICAL \textit{Sweeping} task, and we see favorable performance improvements when we do self-supervised learning of our reward functions in the X-MAGICAL Diverse environment. \textbf{NOTE: Standard $\rightarrow$ Diverse results will be further updated on 6/13.}}
\end{table*}

==> tables/xmagical/cross-emb-same-env.tex <==
\begin{table*}[ht!]
\label{tab:cross-emb-same-env}
\centering
\resizebox{1\textwidth}{!}{%
\begin{tabular}{l|ccc|c}
\multicolumn{1}{c}{} & \multicolumn{3}{c}{} & \multicolumn{1}{c}{} \\
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Standard Env. Pretraining $\rightarrow$ Standard Env. RL} & \multicolumn{1}{c}{} \\
\toprule
Emb. & XIRL & TCN & LIFS & \textbf{GIL} (Ours) \\\midrule
Gripper	& $0.69 \scriptstyle{\pm 0.06}$ & $0.31 \scriptstyle{\pm 0.04}$ & $0.04 \scriptstyle{\pm 0.02}$ & $\mathbf{0.74}$  \\
S-stick & $\mathbf{0.73 \scriptstyle{\pm 0.10}}$ & $0.34 \scriptstyle{\pm 0.05}$ & $0.08 \scriptstyle{\pm 0.02}$ & $0.68$ \\
M-stick & $\mathbf{0.94 \scriptstyle{\pm 0.03}}$ & $0.61 \scriptstyle{\pm 0.03}$ & - &  $0.90$ \\
L-stick & $0.99 \scriptstyle{\pm 0.01}$ & $0.84 \scriptstyle{\pm 0.16}$ & - &  $\mathbf{1.00}$ \\
\bottomrule
\end{tabular}
\hspace{1em}
\begin{tabular}{l|ccc|c}
\multicolumn{1}{c}{} & \multicolumn{3}{c}{} & \multicolumn{1}{c}{} \\
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Diverse Env. Pretraining $\rightarrow$ Diverse Env. RL} & \multicolumn{1}{c}{} \\
\toprule
Emb. & XIRL & TCN & LIFS & \textbf{GIL} (Ours) \\\midrule
Gripper & $\mathbf{0.68 \scriptstyle{\pm 0.10}}$ & $0.00 \scriptstyle{\pm 0.00}$ & - & $0.61$ \\
S-stick &  $\mathbf{0.48 \scriptstyle{\pm 0.08}}$ & $0.00 \scriptstyle{\pm 0.00}$ & $0.00 \scriptstyle{\pm 0.00}$ & $0.45$ \\
M-stick &  $\mathbf{0.88 \scriptstyle{\pm 0.07}}$ & $0.00 \scriptstyle{\pm 0.00}$ & - & $0.84$ \\
L-stick &  $0.73 \scriptstyle{\pm 0.46}$ & $0.00 \scriptstyle{\pm 0.01}$ & $0.01 \scriptstyle{\pm 0.01}$ & $\mathbf{0.87}$ \\
\bottomrule
\end{tabular}
}
\caption{\textit{\textbf{Cross-Embodiment Same-Environment:}} We benchmark the same-environment cross-embodiment performance of XIRL, TCN, and LIFS alongside GIL for the X-MAGICAL \textit{Sweeping} task, and we see favorable performance improvements when we do self-supervised learning of our reward functions in the X-MAGICAL Diverse environment. \textbf{NOTE: results will be further updated on 6/13.}}
\end{table*}

==> tables/xmagical/overview.tex <==
\begin{figure}[t!]
    \centering
    \begin{minipage}{0.9\textwidth}%
        \centering
        \begin{minipage}{0.025\textwidth}
            \centering
            \rotatebox{90}{
                \centering
            Standard~~~~~~~~~~~~~~~~~~~~Diverse~~~~~~
            }
        \end{minipage}\hspace{0.01in}
        \begin{minipage}{0.23\textwidth}
            \centering
            \textbf{Gripper}\vspace{0.005in}\\
            \includegraphics[width=\textwidth]{tables/xmagical/images/diverse-gripper.png}\vspace{0.005in}\\
            \includegraphics[width=\textwidth]{tables/xmagical/images/standard-gripper.png}\vspace{0.01in}\\
        \end{minipage}\hspace{0.01in}
        \begin{minipage}{0.23\textwidth}
            \centering
            \textbf{Short-stick}\vspace{0.03in}\\
            \includegraphics[width=\textwidth]{tables/xmagical/images/diverse-shortstick.png}\vspace{0.005in}\\
            \includegraphics[width=\textwidth]{tables/xmagical/images/standard-shortstick.png}\vspace{0.01in}\\
        \end{minipage}\hspace{0.01in}
        \begin{minipage}{0.23\textwidth}
            \centering
            \textbf{Medium-stick}\vspace{0.03in}\\
            \includegraphics[width=\textwidth]{tables/xmagical/images/diverse-mediumstick.png}\vspace{0.005in}\\
            \includegraphics[width=\textwidth]{tables/xmagical/images/standard-mediumstick.png}\vspace{0.01in}\\
        \end{minipage}\hspace{0.01in}
        \begin{minipage}{0.23\textwidth}
            \centering
            \textbf{Long-stick}\vspace{0.02in}\\
            \includegraphics[width=\textwidth]{tables/xmagical/images/diverse-longstick.png}\vspace{0.005in}\\
            \includegraphics[width=\textwidth]{tables/xmagical/images/standard-longstick.png}\vspace{0.01in}\\
        \end{minipage}
    \end{minipage}\hspace{0.05in}
    \caption{\textbf{Overview of X-MAGICAL task variants.} We consider two environment variants and four embodiments for our simulated sweeping task experiments. Our work assesses the performance of IRL algorithms in both the \textit{Diverse} and \textit{Standard} environments across all four embodiments in the \textit{Same-Embodiment} and \textit{Cross-Embodiment settings}.}
    \label{fig:xmagical-variants}
\end{figure}

==> tables/xmagical/same-emb-cross-env.tex <==
\begin{table*}[ht!]
\label{tab:same-emb-cross-env}
\centering
\resizebox{1\textwidth}{!}{%
\begin{tabular}{l|ccc|c}
\multicolumn{1}{c}{} & \multicolumn{3}{c}{} & \multicolumn{1}{c}{} \\
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Standard Env. Pretraining $\rightarrow$ Diverse Env. RL} & \multicolumn{1}{c}{} \\
\toprule
Emb. & XIRL & TCN & LIFS & \textbf{GIL} (Ours) \\\midrule
Gripper	&  $0.55 \scriptstyle{\pm 0.06}$ & $0.16 \scriptstyle{\pm 0.09}$ & - & $\mathbf{0.62 \scriptstyle{\pm 0.05}}$ \\
S-stick &  $0.22 \scriptstyle{\pm 0.17}$ & $0.39 \scriptstyle{\pm 0.03}$ & - & $\mathbf{0.33 \scriptstyle{\pm 0.06}}$ \\
M-stick & - & $0.44 \scriptstyle{\pm 0.28}$ & - & $0.456 \scriptstyle{\pm 0.06}$ \\
L-stick & $0.75 \scriptstyle{\pm 0.40}$ & - & - & $\mathbf{0.86 \scriptstyle{\pm 0.06}}$ \\
\bottomrule
\end{tabular}
\hspace{1em}
\begin{tabular}{l|ccc|c}
\multicolumn{1}{c}{} & \multicolumn{3}{c}{} & \multicolumn{1}{c}{} \\
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Diverse Env. Pretraining $\rightarrow$ Standard Env. RL} & \multicolumn{1}{c}{} \\
\toprule
Emb. & XIRL & TCN & LIFS & \textbf{GIL} (Ours) \\\midrule
Gripper	& $0.50 \scriptstyle{\pm 0.04}$ & - & - & $\mathbf{0.50 \scriptstyle{\pm 0.03}} $ \\
S-stick &  $0.48 \scriptstyle{\pm 0.11}$ & $0.16 \scriptstyle{\pm 0.15}$ & $0.25 \scriptstyle{\pm 0.04}$ & $\mathbf{0.73 \scriptstyle{\pm 0.02}}$ \\
M-stick &  $\mathbf{0.92 \scriptstyle{\pm 0.05}}$ & $0.01 \scriptstyle{\pm 0.00}$ & $0.00 \scriptstyle{\pm 0.01}$ & $0.87 \scriptstyle{\pm 0.06}$ \\
L-stick &  $0.93 \scriptstyle{\pm 0.08}$ & $0.17 \scriptstyle{\pm 0.10}$ & $0.17 \scriptstyle{\pm 0.11}$ & $\mathbf{0.98 \scriptstyle{\pm 0.02}}$ \\
\bottomrule
\end{tabular}
}
\caption{\textit{\textbf{Same-Embodiment Cross-Environment:}} We benchmark the cross-environment same-embodiment performance of XIRL, TCN, and LIFS alongside GIL for the X-MAGICAL \textit{Sweeping} task, and we see favorable performance improvements when we do self-supervised learning of our reward functions in the X-MAGICAL Diverse environment. \textbf{NOTE: results will be further updated on 6/13.}}
\end{table*}

==> tables/xmagical/xmagical-template.tex <==
\begin{table*}[ht!]
\label{tab:planet}
\vspace{0.05in}
\centering
\resizebox{1\textwidth}{!}{%

\begin{tabular}{l|ccc|c}
\multicolumn{1}{c}{} & \multicolumn{3}{c}{} & \multicolumn{1}{c}{} \\
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Standard Env. Pretraining $\rightarrow$ Diverse Env. RL} & \multicolumn{1}{c}{} \\
\toprule
Embodiment & XIRL & TCN & LIFS & \textbf{GIL} (Ours) \\\midrule
Gripper  & - & - & - & - \\
Short-stick  & - & - & - & - \\
Medium-stick  & - & - & - & - \\
Long-stick  & - & - & - & - \\
\bottomrule
\end{tabular}
\hspace{1em}
\begin{tabular}{l|ccc|c}
\multicolumn{1}{c}{} & \multicolumn{3}{c}{} & \multicolumn{1}{c}{} \\
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Diverse Env. Pretraining $\rightarrow$ Standard Env. RL} & \multicolumn{1}{c}{} \\
\toprule
Embodiment & XIRL & TCN & LIFS & \textbf{GIL} (Ours) \\\midrule
Gripper  & - & - & - & - \\
Short-stick  & - & - & - & - \\
Medium-stick  & - & - & - & - \\
Long-stick  & - & - & - & - \\
\bottomrule
\end{tabular}
}
\caption{\textit{\textbf{Cross-Embodiment Cross-Environment:}} We benchmark the cross-environment cross-embodiment performance of XIRL, TCN, and LIFS alongside GIL for the X-MAGICAL \textit{Sweeping} task, and we see favorable performance improvements when we do self-supervised learning of our reward functions in the X-MAGICAL Diverse environment. [TODO: Update Success Rates]}
\vspace{-0.1in}
\end{table*}
